Controller Synthesis with Inductive Proofs for Piecewise Linear Systems: an SMT-based Algorithm

We present a controller synthesis algorithm for reach-avoid problems for piecewise linear discrete-time systems. Our algorithm relies on SMT solvers and in this paper we focus on piecewise constant control strategies. Our algorithm generates feedback control laws together with inductive proofs of unbounded time safety and progress properties with respect to the reach-avoid sets. Under a reasonable robustness assump- tion, the algorithm is shown to be complete. That is, it either generates a controller of the above type along with a proof of correctness, or it establishes the impossibility of the existence of such controllers. To achieve this, the algorithm iteratively attempts to solve a weakened and strengthened versions of the SMT encoding of the reach-avoid problem. We present preliminary experimental results on applying this algorithm based on a prototype implementation.

==> Introduction.tex <==
% !TEX root = 0main.tex
\section{Introduction}
\label{sec:intro}
A Satisfiability Modulo Theory (SMT) problem is a classical decision problem in computer science~\cite{CDP97}. It takes as input a logical formula in first-order logic that can involve combinations of background theories, and requires one to decide whether or not the formula has a satisfying solution. 
%
For a bounded time horizon $k$, a simplest SMT problem in Equation~(\ref{eq:exsmt}), for instance, is an encoding of a  search for a sequence of control inputs vectors $u_1, \ldots, u_k$ that drives a discrete time linear open-loop control system from every initial state in the hypercube  $[0,0.1]^n$ to the hypercube $[0.9,1]^n$ in $k$ steps, while always keeping the state inside the hypercube  $[0,1]^n$.
\begin{align}
& \exists \ u_1, \ldots u_k, \forall \ x_0 \in [0,0.1]^n, \forall \ t \in \{1,\ldots,k-1\},  \nonumber \\
& \ \ \mbox{let} \ x_{t+1} = A x_t + B u_t \nonumber \\ 
& \ \ \mbox{such that} \ x_t \in [0,1]^n \ \mbox{and} \  x_k \in [0.9,1]^n. \label{eq:exsmt}
\end{align}
This example has several constraints that are defined in terms of the quantified variables $u_i$ and  $x_i$, numerical constants (including those in the matrices $A$ and $B$), and the background theory of linear real arithmetic. 
%
An SMT solver is a software tool that solves SMT problems by  either giving an assignment to the variables that satisfy all the constraints or by saying that none exists. 
%
Modern SMT solvers routinely handle linear problems with thousands of variables and millions of constraints, so much as they have become the engines for innovation in verification and synthesis for computer software and hardware~\cite{de2008z3,barrett2011cvc4,dutertre2006yices}. 
%
Although many control systems can only be modeled by means of nonlinear arithmetic over the real numbers involving transcendental functions that make the corresponding SMT problems undecidable, the solvers are evolving rapidly and several incorporate approximate decision procedures for nonlinear arithmetic~\cite{gao_dreal:_2013}.
These technological developments motivated us (and others~\cite{saha_automated_2014,nedunuri_smt-based_2014}) to explore SMT-based controller synthesis. 

In this paper, we present an algorithm that uses SMT solvers for synthesizing controllers for discrete time systems. The dynamics of the system is given as a piecewise linear feedback control system.
% SM2ZH: is this clear/make sure this sentence is not misleading 
%
The control requirements are the standard {\em reach-avoid\/} specification~\cite{cardenas2008research,cardenas2009challenges}: a set of states $\goal$ that has to be reached while always staying inside a  $\safe$ set.
% Is that the best/oldest reference for reach avoid problems?

A key  difficulty in using SMT for synthesis, is that the resulting SMT problem has to encode the unrolled dynamics of the system with the unknown controller inputs. In the above simple example, this gave rise to $k$ control input variables and the intermediate states. For more general nonlinear models, the intermediate states cannot be written down in closed form and one has to unroll the over-approximations of the dynamics. This can then lead to overtly conservative answers from the solver.  
We present a technique that avoids this problem by synthesizing the control law together with an inductive proof of its correctness. The proof has two parts: (a) an inductive invariant that implies safety and (b) a ranking function that implies progress. A positive side-effect of this is that it can not only synthesize controllers with understandable correctness proofs, but it can also establish the nonexistence of provably correct controllers (of a certain template). 

% give some more details on this below.
%The rest of the paper is organized in the following way.
In Section~\ref{sec:prelim} we define the system model,  the reach-avoid synthesis problem and a particular notion of robustness of models.
In Section~\ref{sec:rules} we first present a basic SMT encoding of the synthesis problem and then a strengthened and a weakened version this encoding. 
Using these two encodings, in Section~\ref{sec:algorithm} we present the synthesis algorithm, its soundness and relative completeness. 
In Section~\ref{sec:case} we illustrate an application of the algorithm in a vehicle navigation problem and conclude in Section~\ref{sec:conc}.


==> formula.tex <==
%% !TEX root = 0main.tex

\section{Constraint-based Synthesis}
\label{sec:rules}
A major barrier in encoding $\synprob$ as an SMT problem is that the safety and progress requirements are over unbounded time. Moreover, these requirements are stated in terms of the future reachable states of the system and computing that in and on itself is a hard problem. Instead of working with unbounded time reach sets, we address this problem by encoding a set of rules that inductively prove safety and progress of the control system.

\subsection{Inductive Synthesis Rules}
\label{ssec:indrules}

In addition to searching for the feedback control law $\vu:\C\rightarrow \U$,
the SMT problem will encode the search for 
(a) an inductive invariant $Inv \subseteq \X$ that proves safety with $\vu$, and 
(b) a ranking function $\V$ that proves progress with $\vu$. 
%

In order to constrain the search, we will fix a {\em template\/} for the ranking function.
%
For this paper, we will use the template $\C\rightarrow \naturals$, that is, any 
function that is piecewise constant on the partition of the state space $\C$. 
%
This choice has an easy interpretation: each entry in the \CPar{} gives the rank of the controller along with the feedback law.
%
Let $\V$ denote the countable set of all such functions. 
%We require the user to provide a {\em template of ranking functions} $\V\subseteq \{V:\X\rightarrow\naturals\}$ that  captures high-level intuitions about how the system progress towards the goal.
Each ranking function $V\in\V$ maps every state in $\X$ to a natural number.
For any $C\in \C$, $V(C)$ is the natural number that all the states $x \in C$ map to.
%In our case studies, we use a template of piecewise constant ranking functions 
%$\V=\{V:\C\rightarrow \naturals\}$, while our proposed method can also incorporate 
%other classes of templates such as $\ell_1$ distance to the goal set or Lyapunov-like functions.
%
Now we are ready to present the basic rules encoding inductive synthesis of $\synprob$:
%%%%%template in V
\begin{figure}[H]
\fbox{\parbox{.9\textwidth}{
\noindent
Find $\vu:\C\rightarrow \U$,  $V\in \V$, $Inv\subseteq \X$ such that: \\
\begin{tabular}{llcl}
R1:&$\init \subseteq Inv$ \\
R2:&$\pst{}{Inv} \subseteq Inv$ \\
R3:&$Inv \subseteq \safe$ \\
R4:&$C\subseteq \goal  \Longleftrightarrow  V(C)=0 $\\
R5:&$C\subseteq Inv \wedge \pst{}{C}\cap C' \neq \emptyset $\\
  & $\quad \Rightarrow V(C) \geq V(C')$\\
R6:&$C\subseteq Inv\backslash \goal  \wedge \pst{k}{C} \cap C'\neq \emptyset$ \\ 
 &  $\quad \implies V(C)>V(C')  $.
\end{tabular}
}
}
\caption{Basic rules $\Pi(M,\C,\V)$ for synthesis for $\synprob$.}
\label{fig:rules}
\end{figure} 
%
%%%% no template
%\begin{figure}[H]
%Find functions $\vu:\C\rightarrow \U$,  $V:\X\rightarrow \naturals$,   $Inv\subseteq \X$ s.t.: 
%\begin{tabular}{llcl}
%R1:& $ \init \subseteq Inv$ \\
%R2:& $post_\vu(Inv) \subseteq Inv$ \\
%R3:&	$ Inv \subseteq \safe$ \\
%R4:&	$x\in \goal  \Longleftrightarrow  V(x)=0 $\\
%R5:& $x\in Inv \implies V(x) \geq V(post_\vu(x))$\\
%R6:&	$x\in Inv\backslash \goal  \implies V(x)>V(post_\vu(x,k))  $
%\end{tabular}
%\caption{Synthesis Rules for $\synprob$}
%\label{fig:rules}
%\end{figure} 
Rules R1-R3 imply that $Inv$ is a fixed-point of $post$ with control $\vu$ that contains 
$\init$ and is contained in $\safe$, and therefore, is adequate for proving safety. 
%l set, which is the exact set of states the system can visit from $\init$ with control $\vu$. 
%R3 encodes the safety condition.
Rule R4 states the the rank of any region $C$ vanishes iff it is in $\goal$. 
Rule R5 encodes  the (Lyapunov-like) property that the rank of any region $C$ is nonincreasing along trajectories. 
Finally, rule R6 states that for any non-$\goal$ region $C$, the rank decreases with $\vu$ within $k$ steps, 
where $k$ is an induction parameter of this encoding.
%
For $\synprob$ specified by model $M$ with $\CPar{}$ $\C$ and a template $\V$, we denote the SMT problem  (Figure~\ref{fig:rules}) as $\Pi(M,\C,\V)$
For some control  $\vu$, ranking function $V\in \V$ and $Inv\subseteq \X$, 
we write \solveorigin{\vu,V,Inv}\footnote{For the sake of clarity, we supress the dependence on $k$.} if the Rules R1-R6 are satisfied.
% if $\vu,V,Inv$.

%We will use a bounded {\em look ahead interval} $k$ which bounds the maximum depth of search such that the ranking function has to decrease.


%To eliminate the quantifiers, 
%we create two uninterpreted functions to amend the synthesis,
%where the {\em invariant set} $Inv$ is the set of states that can be visited by the system under control $\vu$, and $V$ is a discrete type Lyapunov function.
%We thus construct a set of quantifier-free constraints which solve
%the $\synprob$ as shown in Figure~\ref{fig:rules}.
 

 %\begin{figure}[H]
%Find $\vu:\K\rightarrow \U$,  $V:\K\rightarrow \naturals$ and $Inv\subseteq \X$ such that: 
%\begin{tabular}{ll}
%R1:& $ \init \subseteq Inv$ \\
%R2:& $post_\vu(Inv) \subseteq Inv$ \\
%R3:&	$ Inv \subseteq \safe$ \\
%R4:&	$\bigwedge\limits_{C\in \P}( C\subseteq \goal  \Longleftrightarrow  V(C)=0 )$\\
%R5:& $\bigwedge\limits_{C,C'\in \P}(post_\vu(C)\cap C' \neq \emptyset \implies V(C) > V(C'))$\\
%R6:&	$\bigwedge\limits_{C,C'\in \P} (C\subseteq Inv\backslash \goal \implies   post_\vu(C,k))\cap C = \emptyset$.
%\end{tabular}
%\caption{ Synthesis Rules for $\synprob$}
%\label{fig:rules}
%\end{figure}
%\subsection{Soundness of the Synthesis Rules}

%The set of rules R1-R6 in Figure~\ref{fig:rules} is sound. 
%That is, it a control $\vu$ alone with its proof $V,Inv$ 
%satisfy R1-R6, then $\vu$ solves the corresponding $\synprob$.
\begin{theorem}[Soundness]
\label{thm:soundrules}
If \solveorigin{\vu,V,Inv}, then $\vu$ solves $\synprob$ specified by $M$.
\end{theorem}
\begin{proof}
Let $\vu,V,Inv$ satisfy rules in Figure~\eqref{fig:rules}.
Fixing any $x\in \init$, we prove safety and progress conditions separately.

From R1, $x\in Inv$. Combined with R2, we have for any 
$t\in \naturals$, $post_\vu(x,t)\in Inv$.
Since $Inv\subseteq \safe$ (R3) we have $post_\vu(x,t)\in \safe$ for any $t$. Thus the safety condition holds.

We assume $x\in C$ such that $C\cap\goal = \emptyset$; otherwise the progress condition holds trivially.
From R4 we have $V(C)>0$. From R5 and R6,  in at most $kV(C)$ steps,
$V$ decreases to 0. By $R4$ this implies that $x$ reaches the goal.
\end{proof}


\paragraph{Robustness Modulo Templates}

In Section~\ref{sec:model} we defined perturbations of system models,
here we lift the definition to the corresponding synthesis rules:
$\Pi(M',\C',\V')$ is an {\em $\epsilon$-perturbation} of $\Pi(M,\C,\V)$ 
if (i) the $\CPar{}$ and the ranking templates are identical $\C=\C', \V=\V'$,  and 
(ii) the model $M'\in \B_\epsilon(M)$ is an $\epsilon$-perturbation of $M$.

%The synthesis rules R1-R6 are encoded with a template of ranking functions $\V$. 
%With the definition of perturbation of a $\synprob$ $\Pi$,
%we will define robustness of the $\synprob$ $\Pi(M)$ modulo the template $\V$.

\begin{definition}
\label{def:robust}
For a $\CPar{}$ $\C$  and a template of ranking functions $\V$, a $\synprob$ specified by $M$ is {\em robust} modulo $(\C,\V)$ 
if there exists $\epsilon>0$ such that either of the following holds:
\begin{enumerate}[(i)]
\item there exists a control $\vu$ and a ranking function $V\in\V$ such that for any $M'\in \B_\epsilon(M)$, 
\solveoriginprime{\vu,V,Inv}{'} with some $Inv\subseteq \X$, or
\item for none of $M'\in \B_\epsilon(M)$, the synthesis problem $\Pi(M',\C,\V)$ is satisfiable.
\end{enumerate}
\end{definition}
In Theorem~\ref{thm:main} we will show that  our synthesis algorithm is also relatively complete with respect to this notion of robustness. 


%\begin{theorem}
%If there exists a $\vu$ solves $\synprob$, then there exists sufficiently large $k$ and $V,Inv$
%satisfy rules in Figure~\eqref{fig:rules}.
%\end{theorem}
%\begin{proof}
%\end{proof}


%\subsection{Template-based Construction of $Inv,V$}
%\label{sec:template}
%
%The rules in Figure~\ref{fig:rules} are
%practically solved with help from user-provided templates that capture high-level intuitions about the control.
%
%In this work, the functions $Inv,V$ are interpreted as piece-wise constant functions.
%require the user to provide a finite partition $\P$ of  the state space 
%which preserves $\init,\safe,\goal$.
%Then the partition $\P$  specifies a class of $\vu,Inv,V$ to search for:
%
%Roughly, the system is oblivious of states in the same cell $C\in \P$.
%Thus, the Lyapunov function as a
%function maps each cell to an integer.
%Similarly, the invariant is captured by a function $Inv:\P\rightarrow \{0,1\}$ such that 
%a cell returns 1 iff it is contained by $Inv$.
%In the next section, we rewrite Figure~\ref{fig:rules} with this template.




\subsection{Weakened and Strengthened Rules}
\label{ssec:relaxed} 

The main challenge in solving $\Pi(M,\C,\V)$ is the $post$ operator in Rules R2, R5, and R6. 
We need a reasonable representation of $post$ for this computation to be effective. 
In this work,  we use a finite partition $\P$ of the state space (which preserves $\C,\init,\safe,\goal$)
for computing the $post$. This choices is somewhat independent of the rest of the methodology
and any other template (for example, linear functions, support functions, zonotopes) could be used instead of the fixed partitions. 

%Then set $Inv$ is interpreted as a finite union of cells in $\P$.


%The invariant $Inv$ are practically solved with help from user-provided templates. \\

%For a cell $P\in \P$, the post operator of $P$ ($post_\vu(P)$)  
%may not be able to compute precisely. 
%Moreover, $post_\vu(P)$ may not be preserved by $\P$. 
%These two factors  prevent precise encoding the rules in Figure~\ref{fig:rules}.
The key idea to solve it is to create  {\em over} and  {\em under} approximations of the $post$ operator with respect to the representation of choice---in this case representation using the fixed partition $\P$.
These operators are then used to create weakened and strengthened versions of the basic inductive rules that can be effectively solved as SMT problems. 

We define an over-approximation ($\P\text{-}\overline{post}$) and an under-approximation  ($\P\text{-}\underline{post}$) of the $post$ operator with respect to a partition $\P$ as follows: for any compact $S\subseteq \X$,
\begin{eqnarray}
\label{eq:wpst}
\wpst{}{S}\P &=& \bigcup\limits_{P\in \P \wedge P\cap \pst{}{S} \neq \emptyset}P,\\
\label{eq:npst}
\npst{}{S}\P &=& \bigcup\limits_{P\in \P \wedge P\subseteq \pst{}{S}}P.
\end{eqnarray}
Roughly, the over-approximation  $\wpst{}{S}\P$ computes the minimum superset of $S$ which is preserved by $\P$ and the under-approximation  $\npst{}{S}\P$ computes the maximum subset of $S$ which is preserved by $\P$.  
%The $\wpst{}{S}\P$ and $\npst{}{S}\P$ are discrete operators which are assumed to be computed precisely.
We define $\wpst{t}{S}\P$ and $\npst{t}{S}\P$ as the $t$ step over and under-approximations in the usual way.

%\mitras{will resume here.}
\begin{prop}
\label{prop:complete}
For any measurable $S\subseteq \X$, a $post$ operator and any partition $\P$, the following properties hold:
\begin{enumerate}[(i)]
\item $\npst{}{S}\P \subseteq \pst{}{S} \subseteq \wpst{}{S}\P$, 

\item If $\P'$ subsumes $\P$, then $\npst{}{S}{\P'}\supseteq \npst{}{S}{\P}$ and $\wpst{}{S}{\P'}\subseteq \wpst{}{S}{\P}$, and

\item For any $\epsilon>0$,  
$\exists \ \delta>0$ such that for any $\P$ with resolution less than $\delta$,
$d(\npst{}{S}\P,\wpst{}{S}\P)<\epsilon$.
\end{enumerate}
\end{prop}

Instead of searching for an exact inductive invariant $Inv$, the weakened and strengthened versions of the synthesis rules presented below try to find under ($Must$) and over-approximations ($May$) of the invariant using the $\wpst{}{S}\P$ and $\npst{}{S}\P$ operators. 
\begin{figure}[ht]
\fbox{\parbox{0.9\textwidth}{

Find $\vu:\C\rightarrow \U$,  $V\in \V$, $\must\subseteq \X$ such that   \\
\begin{tabular}{ll}
%R0:& $ Must \subseteq \may$\\
W1:& $ \init \subseteq \must $\\
W2:& $ \npst{}{\must}\P \subseteq \must $\\
W3:&	$ \must\subseteq \safe$ \\
W4:&	$C\subseteq \goal  \Longleftrightarrow  V(C)=0 $\\
W5:& $C\subseteq \must \wedge C'\subseteq \npst{}{C}\P $\\
& $\ \implies V(C) \geq V(C')$\\
W6:&	$C\subseteq \must\backslash \goal  \wedge C'\subseteq \npst{k}{C}\P$\\
  	&  $\ \implies V(C)>V(C') $
\end{tabular}
}}
\caption{ Weakened rules $\Pi_\P^w(M,\C,\V)$ for synthesis.}
\label{fig:underrules}
\end{figure}
\begin{figure}[ht]
\fbox{\parbox{.9\textwidth}{
Find $\vu:\C\rightarrow \U$,  $V\in \V$, $\may\subseteq \X$ s.t.: \\
\begin{tabular}{ll}
%R0:& $ Must \subseteq \may$\\
S1:& $ \init \subseteq \may $\\
S2:& $ \wpst{}{\may}\P \subseteq \may $\\
S3:&	$ \may\subseteq \safe$ \\
S4:&	$C\subseteq \goal  \Longleftrightarrow  V(C)=0 $\\
S5:& $C\subseteq \may \wedge C'\subseteq \wpst{}{C}\P $\\
& $\ \implies V(C) \geq V(C')$\\
S6:&	$C\subseteq \may\backslash \goal \wedge  C'\subseteq \wpst{k}{C}\P$\\
  	&  $\ \implies V(C)>V(C') $
\end{tabular}
}}
\caption{Strengthened rules $\Pi_\P^s(M,\C,\V)$ for synthesis.}
\label{fig:overrules}
\end{figure}

%%%% no template for V
%\begin{figure}[H]
%Find $\vu:\C\rightarrow \U$,  $V:\X\rightarrow \naturals$, $\must\subseteq \X$ s.t.: 
%\begin{tabular}{ll}
%%R0:& $ Must \subseteq \may$\\
%R1:& $ \init \subseteq \must$\\
%R2:& $ \npst{}{S}\P(\must) \subseteq \must $\\
%R3:&	$ \must\subseteq \safe$ \\
%R4:&	$P\subseteq \goal  \Longleftrightarrow  V_u(P)=0$\\
%R5:& $P\subseteq \must \implies  V_u(P)\geq (V_u(\npst{}{S}\P(P))$\\
%R6:&	$P\subseteq \must\backslash \goal \implies V_u(C) < V_u(\npst{}{S}\P(C,k))$
%\end{tabular}
%\caption{ Relaxed Rules for $\synprob$}
%\label{fig:underrules}
%\end{figure}
%%% with template for V


%\begin{figure}[H]
%Find $\vu:\C\rightarrow \U$,  $V:\C\rightarrow \naturals$, $\may\subseteq \X$ s.t.: 
%\begin{tabular}{ll}
%%R0:& $ Must \subseteq \may$\\
%R1:& $ \init \subseteq \may $\\
%R2:& $ \wpst{}{S}\P(\may) \subseteq \may $\\
%R3:&	$ \may\subseteq \safe$ \\
%R4:&	$P\subseteq \goal  \Longleftrightarrow  V_u(P)=0$\\
%R5:& $P\subseteq \may  \implies  V_l(P)\geq V_u(\wpst{}{S}\P(P)) $\\
%R6:&	$P\subseteq \may \backslash \goal \implies V_u(C) < V_u(\wpst{}{S}\P(C,k))$
%\end{tabular}
%\caption{ Strenthened Rules for $\synprob$}
%\label{fig:overrules}
%\end{figure}

% We do not have to define this again.
%We write  \solveunder{\vu,V,\must} if $\vu,V,\must$ satisfy the weakened rules W1-W6 and \solveover{\vu,V,\may} if they satisfy the set of strengthened rules in Figure~\ref{fig:overrules}.

%\begin{lemma}[Relaxation and Strenthening]
%If the strengthened rules (Figure~\ref{fig:overrules}) are solvable, then the original rules (Figure~\ref{fig:rules}) are solvable.
%If the relaxed rules (Figure~\ref{fig:underrules}) are unsatisfiable, the original rules (Figure~\ref{fig:rules}) are unsatisfiable
%\end{lemma}
\begin{lemma}
\label{lem:sound}
For any $\P$, the  following hold:
\begin{enumerate}[(i)] 
\item if \solveorigin{\vu,V,Inv}, then there exist $\must\subseteq \X$ such that \solveunder{\vu,V,\must}; 
and 
\item if \solveover{\vu,V,\may}, then exists $Inv\subseteq \X$ such that \solveorigin{\vu,V,Inv}.
\end{enumerate}
\end{lemma}
\begin{proof}
Suppose \solveorigin{\vu,V,Inv}. We will show that there exists a $\must\subseteq \X$
satisfying the weakened rules (W1-W6).
Fix a $\vu$. From Proposition~\ref{prop:complete}, the operator $\npst{}{\cdot}\P$ is upper bounded by 
$\pst{}{\cdot}$.
Since  $\pst{}{\cdot}$ has a fixed point $Inv$,
the fixed point of
$\npst{}{S}\P$ exists.
Let $\must$ be  the fixed point defined by W1-W2 and we have $\must \subseteq Inv$.
It follows that $\must\subseteq Inv\subseteq \safe$ and W3 holds.
W4 is inherited from  R4.
For any $C\subseteq \must \wedge C'\subseteq \npst{}{S}\P(C)$,
we have $\may\subseteq Inv$ and $\npst{}{S}\P(C)\subseteq post_\vu(C)$.
From R5, therefore,  $V(C)\geq V(C')$ and W5 holds.
Similarly, $\npst{}{S}\P(C,k)\subseteq post_\vu(C,k)$, thus W6 also holds.
Therefore, \solveunder{\vu,V,\must}.

The proof of second part is similar. 
%the existence of $Inv$ such that \solveorigin{\vu,V,Inv} is similar.
\end{proof}








==> method.tex <==
%% !TEX root = 0main.tex
\section{Annotation-based Reachability}

\subsection{Discrepancy and Approximations}
First of all, we will use the definition of discrepancy function~\cite{HuangM:HSCC2014}, which enables us to use annotations to check invariants of the composed system. The discrepancy function for a location $l$ of $\A$ (or for a dynamical system) bounds the distance between two trajectories in location $l$ from different initial states, as a function of time and the inputs they receive.
\begin{definition}
\label{def:discrep}
For a $\A$, a continuous function $V:\X^2  \mapsto \nnreals$ is an {\em discrepancy function\/}
for a location $\ell$ if
\begin{enumerate}[(a)]
%\item $x_1 = x_2 \Leftrightarrow V(x_1,x_2) = 0$,
\item $\exists$ class-$\K$ functions (see \cite{HuangM:HSCC2014}) $\lalpha,\ualpha$, s.t., $\forall  x,x'\in \X$, $\lalpha(|x-x'|)\leq V(x,x') \leq \ualpha(|x-x'|)$, and
\item $\exists \beta:\nnreals \times [T] \mapsto \nnreals$ such that for any $x,x'\in \X$, any input trajectories $\vu$:
$\U^T$, and any $t\in[T]$,
\[
\begin{array}{c}
V(\xi(x,\vu,t),\xi(x',\vu,t)) \leq  \beta(|x - x'|,t).
\end{array}
\] 
In addition, $\beta(\cdot,\cdot)$ is of class-$\K$ in the first argument.
\end{enumerate}
\end{definition}
The tuple $(\lalpha,\ualpha, \beta,\gamma)$ is called the {\em witness} of the discrepancy function $V$.
The first condition merely bounds $V$ in terms of the norm of its arguments.
The more important second condition ensures that the distance between the trajectories is bounded as a function of $\beta$, and can be reduced arbitrarily
by making $x \arrow{} x'$.
%











